On Optimal Caching and Model Multiplexing for Large Model Inference

Large Language Models (LLMs) and other large foundation models have achieved noteworthy success, but their size exacerbates existing resource consumption and latency challenges. In particular, the large-scale deployment of these models is hindered by the significant resource requirements during inference. In this paper, we study two approaches for mitigating these challenges: employing a cache to store previous queries and learning a model multiplexer to choose from an ensemble of models for query processing. Theoretically, we provide an optimal algorithm for jointly optimizing both approaches to reduce the inference cost in both offline and online tabular settings. By combining a caching algorithm, namely Greedy Dual Size with Frequency (GDSF) or Least Expected Cost (LEC), with a model multiplexer, we achieve optimal rates in both offline and online settings. Empirically, simulations show that the combination of our caching and model multiplexing algorithms greatly improves over the baselines, with up to $50\times$ improvement over the baseline when the ratio between the maximum cost and minimum cost is $100$. Experiments on real datasets show a $4.3\times$ improvement in FLOPs over the baseline when the ratio for FLOPs is $10$, and a $1.8\times$ improvement in latency when the ratio for average latency is $1.85$.

==> tables/q100r10000c40/offline_oasst_fastchat-t5_vicuna.tex <==
\begin{table}[ht]
\begin{center}
\begin{tabular}{ cp{3.5em}p{3.2em}p{3.2em}p{3.2em}p{3.2em}p{3.2em}p{3.2em} }
  \toprule
  $\alpha$ & selector accuracy & LFU+ large & LFU+ cascade & LFU+ selector & LEC+ large & LEC+ cascade & LEC+ selector \\
  \midrule
  0.2 & \multicolumn{1}{r}{ 0.8 } & \multicolumn{1}{r}{ 8.47 } & \multicolumn{1}{r}{ 12.35 } & \multicolumn{1}{r}{ 8.03 } & \multicolumn{1}{r}{ 7.98 } & \multicolumn{1}{r}{ 7.27 } & \multicolumn{1}{r}{ \textbf{ 7.04 } } \\
  0.5 & \multicolumn{1}{r}{ 0.8 } & \multicolumn{1}{r}{ 19.19 } & \multicolumn{1}{r}{ 28.94 } & \multicolumn{1}{r}{ 17.89 } & \multicolumn{1}{r}{ 17.58 } & \multicolumn{1}{r}{ 15.25 } & \multicolumn{1}{r}{ \textbf{ 14.47 } } \\
  0.8 & \multicolumn{1}{r}{ 0.8 } & \multicolumn{1}{r}{ 26.42 } & \multicolumn{1}{r}{ 40.95 } & \multicolumn{1}{r}{ 25.52 } & \multicolumn{1}{r}{ 24.57 } & \multicolumn{1}{r}{ 18.68 } & \multicolumn{1}{r}{ \textbf{ 18.22 } } \\
  \midrule
  0.2 & \multicolumn{1}{r}{ 1 } & \multicolumn{1}{r}{ 8.68 } & \multicolumn{1}{r}{ 12.93 } & \multicolumn{1}{r}{ 6.50 } & \multicolumn{1}{r}{ 7.87 } & \multicolumn{1}{r}{ 7.83 } & \multicolumn{1}{r}{ \textbf{ 4.93 } } \\
  0.5 & \multicolumn{1}{r}{ 1 } & \multicolumn{1}{r}{ 19.52 } & \multicolumn{1}{r}{ 27.94 } & \multicolumn{1}{r}{ 13.39 } & \multicolumn{1}{r}{ 17.73 } & \multicolumn{1}{r}{ 16.03 } & \multicolumn{1}{r}{ \textbf{ 10.37 } } \\
  0.8 & \multicolumn{1}{r}{ 1 } & \multicolumn{1}{r}{ 26.88 } & \multicolumn{1}{r}{ 39.06 } & \multicolumn{1}{r}{ 19.28 } & \multicolumn{1}{r}{ 24.70 } & \multicolumn{1}{r}{ 19.30 } & \multicolumn{1}{r}{ \textbf{ 13.91 } } \\
  \bottomrule
\end{tabular}
\end{center}
\caption{Latency for offline oasst, fastchat-t5 vs vicuna}
\label{tab:offline_oasst_fastchat-t5_vicuna}
\end{table}

==> tables/q100r10000c40/offline_oasst_flan-t5_vicuna.tex <==
\begin{table}[ht]
\begin{center}
\begin{tabular}{ cp{3.5em}p{3.1em}p{3.1em}p{3.1em}p{3.1em}p{3.1em}p{3.1em} }
  \toprule
  $\alpha$ & selector accuracy & LFU+ large & LFU+ cascade & LFU+ selector & LEC+ large & LEC+ cascade & LEC+ selector \\ 
  \bottomrule
\end{tabular}
\end{center}
\caption{offline oasst flan-t5 vicuna}
\label{tab:offline_oasst_flan-t5_vicuna}
\end{table}


==> tables/q100r10000c40/online_lambda_opt-1.3b_opt-13b.tex <==
\begin{table}[ht]
\begin{center}
\begin{tabular}{ cp{3.2em}p{3.2em}p{3.2em}p{3.2em}p{3.2em}p{3.2em} }
  \toprule
  $\alpha$ &  LFU+ large & LFU+ cascade & LFU+ selector & LEC+ large & LEC+ cascade & LEC+ selector \\
  \midrule
  0.2 & \multicolumn{1}{r}{ 3.82 } & \multicolumn{1}{r}{ 3.82 } & \multicolumn{1}{r}{ 2.23 } & \multicolumn{1}{r}{ 3.72 } & \multicolumn{1}{r}{ 1.87 } & \multicolumn{1}{r}{ \textbf{ 1.28 } } \\
  0.8 & \multicolumn{1}{r}{ 11.33 } & \multicolumn{1}{r}{ 12.88 } & \multicolumn{1}{r}{ 6.58 } & \multicolumn{1}{r}{ 10.92 } & \multicolumn{1}{r}{ 4.61 } & \multicolumn{1}{r}{ \textbf{ 2.87 } } \\
  \bottomrule
\end{tabular}
\end{center}
\caption{online lambda opt-1.3b opt-13b}
\label{tab:online_lambda_opt-1.3b_opt-13b}
\end{table}

==> tables/q100r10000c40/online_oasst_flan-t5_vicuna.tex <==
\begin{table}[ht]
\begin{center}
\begin{tabular}{ cp{3.1em}p{3.1em}p{3.1em}p{3.1em}p{3.1em}p{3.1em} }
  \toprule
  $\alpha$ &  LFU+ large & LFU+ cascade & LFU+ selector & LEC+ large & LEC+ cascade & LEC+ selector \\ 
  \bottomrule
\end{tabular}
\end{center}
\caption{online oasst flan-t5 vicuna}
\label{tab:online_oasst_flan-t5_vicuna}
\end{table}

